Characterizing the Low-Redshift Intergalactic Medium towards PKS1302-102

We present a detailed analysis of the intergalactic metal-line absorption systems in the archival HST/STIS and FUSE ultraviolet spectra of the low-redshift quasar PKS1302-102 (z_QSO = 0.2784). We supplement the archive data with CLOUDY ionization models and a survey of galaxies in the quasar field. There are 15 strong Lya absorbers with column densities logN_HI > 14. Of these, six are associated with at least CIII 977 absorption (logN(C^++) > 13); this implies a redshift density dN_CIII/dz = 36+13/-9 (68% confidence limits) for the five detections with rest equivalent width W_r > 50 mA. Two systems show OVI 1031,1037 absorption in addition to CIII (logN(O^+5) > 14). One is a partial Lyman limit system (logN_HI = 17) with associated CIII, OVI, and SiIII 1206 absorption. There are three tentative OVI systems that do not have CIII detected. For one OVI doublet with both lines detected at 3 sigma with W_r > 50 mA, dN_OVI/dz = 7+9/-4. We also search for OVI doublets without Lya absorption but identify none. From CLOUDY modeling, these metal-line systems have metallicities spanning the range -4 < [M/H] < -0.3. The two OVI systems with associated CIII absorption cannot be single-phase, collisionally-ionized media based on the relative abundances of the metals and kinematic arguments. From the galaxy survey, we discover that the absorption systems are in a diverse set of galactic environments. Each metal-line system has at least one galaxy within 500 km/s and 600 h^-1 kpc with L > 0.1 L_*.

==> tab2_online.tex <==
 
\clearpage
 
\begin{deluxetable}{lccrcccccc}
\tablewidth{0pc}
\tablecaption{$W_{r}$ SUMMARY \label{tab:ewsumm}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Ion} & \colhead{$\lambda_{obs}$} &\colhead{$\lambda_{r}$} & \colhead{$z_{abs}$} & \colhead{$W_1$} 
& \colhead{$\sigma(W_1)$}& \colhead{$W_2$} & \colhead{$\sigma(W_2)$} &
\colhead{$W_f$} & \colhead{$\sigma(W_f)$} \\
 & (\AA) & (\AA) && (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA)} 
\startdata
\cutinhead{\emph{FUSE}}
\ion{H}{1} 930& 934.798& 930.748& 0.00435&$ 168$&$ 47$&$  74$&$ 37$&$ 110$& 29\\
\ion{H}{1} 937& 941.898& 937.803& 0.00437&$ 293$&$ 60$&$ 247$&$ 40$&$ 262$& 33\\
\ion{O}{1} 948& 948.654& 948.686&-0.00003&$ 424$&$ 53$& \nodata & \nodata &$ 424$& 53\\
\ion{O}{1} 950& 950.976& 950.885& 0.00010&$ 211$&$ 41$& \nodata & \nodata &$ 211$& 41\\
\ion{N}{1} 953a& 953.366& 953.415&-0.00005&$ 178$&$ 33$& \nodata & \nodata &$ 178$& 33\\
\ion{N}{1} 953b& 953.632& 953.655&-0.00002&$ 306$&$ 32$& \nodata & \nodata &$ 306$& 32\\
\ion{N}{1} 953c& 953.981& 953.970& 0.00001&$ 322$&$ 38$& \nodata & \nodata &$ 322$& 38\\
\ion{H}{1} 949& 953.995& 949.743& 0.00448&$ 418$&$ 68$&$ 305$&$ 38$&$ 332$& 33\\
\ion{P}{2} 963& 963.804& 963.801& 0.00000&$ 388$&$ 63$& \nodata & \nodata &$ 388$& 63\\
H$_2$& 965.023& 964.981& 0.00004&$ 156$&$ 49$& \nodata & \nodata &$ 156$& 49\\
\ion{O}{1} 971& 971.719& 971.738&-0.00002&$ 228$&$ 43$& \nodata & \nodata &$ 228$& 43\\
H$_2$& 972.172& 971.985& 0.00019&$ 259$&$ 33$& \nodata & \nodata &$ 259$& 33\\
\ion{H}{1} 972& 976.903& 972.537& 0.00449&$ 367$&$ 86$&$ 350$&$ 44$&$ 353$& 39\\
\ion{C}{3} 977& 976.926& 977.020&-0.00010&$ 391$&$ 45$& \nodata & \nodata &$ 391$& 45\\
\ion{H}{1} 937& 977.333& 937.803& 0.04215&$   7$&$ 74$&$  15$&$ 44$&$  13$& 38\\
H$_2$& 981.309& 981.437&-0.00013&$ 150$&$ 44$& \nodata & \nodata &$ 150$& 44\\
\ion{C}{3} 977& 981.309& 977.020& 0.00439&$   7$&$ 63$&$ 156$&$ 41$&$ 111$& 35\\
\ion{N}{3} 989& 989.770& 989.799&-0.00003&$ 603$&$ 41$& \nodata & \nodata &$ 603$& 41\\
\ion{Si}{2} 989& 989.770& 989.873&-0.00010&$ 603$&$ 41$& \nodata & \nodata &$ 603$& 41\\
\ion{H}{1} 949& 989.770& 949.743& 0.04214&$ 349$&$ 81$&$ 584$&$ 37$&$ 542$& 34\\
\ion{H}{1} 914a&1000.712& 914.039& 0.09482&$  68$&$ 20$& \nodata & \nodata &$  68$& 20\\
\ion{H}{1} 914b&1000.998& 914.286& 0.09484&$  64$&$ 17$& \nodata & \nodata &$  64$& 17\\
\ion{H}{1} 914c&1001.290& 914.576& 0.09481&$ 129$&$ 19$& \nodata & \nodata &$ 129$& 19\\
H$_2$&1001.660&1001.652& 0.00001&$ 170$&$ 38$& \nodata & \nodata &$ 170$& 38\\
H$_2$&1001.782&1001.821&-0.00004&$ 215$&$ 23$& \nodata & \nodata &$ 215$& 23\\
\ion{H}{1} 914d&1001.782& 914.919& 0.09494&$ 189$&$ 18$& \nodata & \nodata &$ 189$& 18\\
\ion{H}{1} 915a&1002.155& 915.329& 0.09486&$ 173$&$ 17$& \nodata & \nodata &$ 173$& 17\\
H$_2$&1002.428&1002.449&-0.00002&$ 147$&$ 26$&$ 149$&$ 17$&$ 148$& 14\\
\ion{H}{1} 915b&1002.653& 915.824& 0.09481&$ 180$&$ 14$& \nodata & \nodata &$ 180$& 14\\
H$_2$&1003.339&1003.294& 0.00005&$ 163$&$ 44$&$ 236$&$ 20$&$ 238$& 16\\
\ion{H}{1} 916&1003.339& 916.429& 0.09484&$ 217$&$ 18$& \nodata & \nodata &$ 217$& 18\\
H$_2$&1003.966&1003.982&-0.00002&$  45$&$ 16$&$ 329$&$ 21$&$ 132$& 11\\
\ion{H}{1} 917&1004.182& 917.181& 0.09486&$ 183$&$ 14$& \nodata & \nodata &$ 183$& 14\\
\ion{H}{1} 918&1005.237& 918.129& 0.09488&$ 215$&$ 11$& \nodata & \nodata &$ 215$& 11\\
H$_2$&1005.335&1005.390&-0.00005&$  50$&$  9$&$  74$&$ 19$&$  57$&  7\\
H$_2$&1006.495&1006.411& 0.00008&$ 288$&$ 16$&$ 369$&$ 39$&$ 293$& 14\\
\ion{H}{1} 919&1006.524& 919.351& 0.09482&$ 263$&$ 15$& \nodata & \nodata &$ 263$& 15\\
\ion{H}{1} 920&1008.346& 920.963& 0.09488&$ 408$&$ 14$& \nodata & \nodata &$ 408$& 14\\
H$_2$&1008.388&1008.552&-0.00016&$ 447$&$ 15$&$ 509$&$ 51$&$ 450$& 13\\
H$_2$&1008.388&1008.383& 0.00001&$ 447$&$ 15$&$ 509$&$ 51$&$ 450$& 13\\
H$_2$&1008.988&1009.024&-0.00004&$  59$&$ 12$&$  17$&$ 41$&$  47$& 11\\
H$_2$&1009.710&1009.771&-0.00006&$ 163$&$ 12$&$ 161$&$ 45$&$ 160$& 11\\
H$_2$&1010.158&1010.129& 0.00003&$  74$&$ 11$&$ -22$&$ 40$&$  62$& 10\\
\ion{H}{1} 923&1010.720& 923.150& 0.09486&$ 360$&$ 13$& \nodata & \nodata &$ 360$& 13\\
H$_2$&1010.736&1010.938&-0.00020&$ 395$&$ 14$&$ 447$&$ 57$&$ 398$& 12\\
H$_2$&1012.065&1012.169&-0.00010&$  81$&$ 14$&$  68$&$ 55$&$  84$& 13\\
\ion{S}{3} 1012&1012.596&1012.502& 0.00009&$ 148$&$ 12$&$ 212$&$ 47$&$ 164$& 11\\
H$_2$&1012.843&1012.810& 0.00003&$  84$&$  8$&$   1$&$ 37$&$  77$&  8\\
H$_2$&1013.399&1013.435&-0.00004&$ 166$&$ 11$&$ 246$&$ 44$&$ 168$& 10\\
\ion{H}{1} 972&1013.613& 972.537& 0.04224&$ 152$&$  9$& \nodata & \nodata &$ 152$&  9\\
\ion{H}{1} 926&1014.076& 926.226& 0.09485&$ 397$&$  9$& \nodata & \nodata &$ 397$&  9\\
H$_2$&1014.150&1014.326&-0.00017&$ 434$&$ 10$&$ 534$&$ 47$&$ 438$&  9\\
H$_2$&1014.500&1014.504&-0.00000&$  36$&$ 11$&$ -23$&$ 43$&$  32$& 11\\
H$_2$&1014.955&1014.974&-0.00002&$  46$&$ 13$&$ -11$&$ 47$&$  42$& 12\\
H$_2$&1016.451&1016.485&-0.00003&$  71$&$ 12$&$  41$&$ 42$&$  68$& 11\\
H$_2$&1017.452&1017.422& 0.00003&$  42$&$ 11$&$  75$&$ 35$&$  45$& 11\\
\ion{C}{3} 977&1018.287& 977.020& 0.04224&$ 168$&$ 12$& \nodata & \nodata &$ 168$& 12\\
\ion{H}{1} 930&1019.019& 930.748& 0.09484&$ 341$&$ 10$& \nodata & \nodata &$ 341$& 10\\
H$_2$&1019.467&1019.500&-0.00003&$  33$&$ 11$&$ -35$&$ 34$&$  26$& 11\\
\ion{Si}{2} 1020&1020.694&1020.699&-0.00000&$ 217$&$ 11$&$ 283$&$ 36$&$ 434$&  2\\
H$_2$&1024.435&1024.372& 0.00006&$ 161$&$ 12$&$ 154$&$ 41$&$ 161$& 11\\
\ion{H}{1} 972&1024.914& 972.537& 0.05386&$ 223$&$ 10$& \nodata & \nodata &$ 223$& 10\\
H$_2$&1024.962&1024.986&-0.00002&$ 181$&$  9$&$ 283$&$ 32$&$ 189$&  8\\
H$_2$&1026.731&1026.526& 0.00020&$ 574$&$ 10$&$ 926$&$ 51$&$ 587$& 10\\
\ion{H}{1} 937&1026.742& 937.803& 0.09484&$ 524$&$  9$& \nodata & \nodata &$ 524$&  9\\
H$_2$&1028.057&1028.103&-0.00004&$  45$&$ 15$&$   9$&$ 51$&$  42$& 14\\
H$_2$&1029.075&1028.985& 0.00009&$  78$&$ 10$&$  -4$&$ 51$&$  74$& 10\\
\ion{H}{1} 1025&1030.228&1025.722& 0.00439&$ 244$&$ 12$& \nodata & \nodata &$ 244$& 12\\
H$_2$&1031.198&1031.191& 0.00001&$  47$&$ 10$&$  88$&$ 44$&$  49$& 10\\
\ion{O}{6} 1031&1031.965&1031.926& 0.00004&$ 199$&$ 13$&$ 215$&$ 61$&$ 193$& 11\\
\ion{H}{1} 972&1035.382& 972.537& 0.06462&$  13$&$ 15$& \nodata & \nodata &$  13$& 15\\
\ion{C}{2} 1036&1036.399&1036.337& 0.00006&$ 426$&$ 13$&$ 712$&$ 68$&$ 462$& 11\\
H$_2$&1037.101&1037.149&-0.00005&$ 146$&$ 14$&$ 357$&$ 61$&$ 156$& 13\\
\ion{O}{6} 1037&1037.612&1037.617&-0.00000&$  96$&$ 13$&$  35$&$ 61$&$ 121$& 11\\
H$_2$&1038.082&1038.157&-0.00007&$  82$&$ 10$&$  64$&$ 47$&$  81$& 10\\
H$_2$&1038.713&1038.689& 0.00002&$  73$&$ 12$&$ 133$&$ 50$&$  76$& 11\\
\ion{O}{1} 1039&1039.149&1039.230&-0.00008&$ 346$&$ 14$&$ 499$&$ 55$&$ 355$& 13\\
\ion{H}{1} 949&1039.251& 949.743& 0.09424&$ 316$&$ 12$& \nodata & \nodata &$ 316$& 12\\
\ion{H}{1} 949&1039.849& 949.743& 0.09487&$ 390$&$ 11$& \nodata & \nodata &$ 390$& 11\\
H$_2$&1040.000&1040.058&-0.00006&$  68$&$  6$&$ 103$&$ 30$&$  70$&  6\\
H$_2$&1040.359&1040.366&-0.00001&$  61$&$  8$&$  49$&$ 37$&$  60$&  8\\
\ion{C}{3} 977&1040.359& 977.020& 0.06483&$  57$&$  8$&$  46$&$ 35$&$  56$&  8\\
H$_2$&1041.166&1041.158& 0.00001&$  20$&$ 11$&$  74$&$ 30$&$  26$& 10\\
H$_2$&1043.387&1043.502&-0.00011&$  81$&$ 15$&$  32$&$ 60$&$  78$& 14\\
\ion{H}{1} 949&1043.729& 949.743& 0.09896&$   7$&$  9$& \nodata & \nodata &$   7$&  9\\
\ion{Ar}{1} 1048&1048.173&1048.220&-0.00004&$ 148$&$ 12$&$ 292$&$ 47$&$ 154$& 10\\
H$_2$&1049.359&1049.367&-0.00001&$  79$&$ 12$&$ 130$&$ 49$&$  82$& 12\\
H$_2$&1049.911&1049.960&-0.00005&$ 139$&$ 14$&$ 144$&$ 59$&$ 139$& 14\\
H$_2$&1051.002&1051.033&-0.00003&$ 102$&$ 14$&$ 135$&$ 55$&$ 104$& 13\\
H$_2$&1051.531&1051.498& 0.00003&$ 120$&$ 13$&$  89$&$ 54$&$ 119$& 12\\
H$_2$&1053.278&1053.284&-0.00001&$  52$&$  8$&$ 106$&$ 30$&$  56$&  8\\
H$_2$&1053.893&1053.976&-0.00008&$  63$&$ 11$&$ 115$&$ 41$&$  66$& 11\\
\ion{Fe}{2} 1055&1055.345&1055.262& 0.00008&$  94$&$ 11$&$  89$&$ 43$&$  80$&  9\\
H$_2$&1056.420&1056.472&-0.00005&$  41$&$  9$&$  70$&$ 36$&$  43$&  9\\
H$_2$&1062.845&1062.882&-0.00004&$  79$&$ 11$&$  -4$&$ 49$&$  75$& 11\\
\ion{Fe}{2} 1063&1063.232&1063.176& 0.00005&$ 243$&$  9$&$ 357$&$ 44$&$ 248$&  8\\
H$_2$&1063.441&1063.460&-0.00002&$  92$&$  7$&$ 151$&$ 30$&$  94$&  6\\
\ion{H}{1} 972&1063.926& 972.537& 0.09397&$ 163$&$ 10$& \nodata & \nodata &$ 163$& 10\\
\ion{Fe}{2} 1064&1063.967&1063.972&-0.00000&$ 178$&$ 11$&$ 169$&$ 53$&$ 189$&  9\\
H$_2$&1064.575&1064.606&-0.00003&$ 148$&$  9$&$ 203$&$ 42$&$ 150$&  8\\
\ion{H}{1} 972&1064.766& 972.537& 0.09483&$ 465$&$ 13$& \nodata & \nodata &$ 465$& 13\\
H$_2$&1064.957&1064.994&-0.00003&$ 107$&$  8$&$ 151$&$ 38$&$ 109$&  8\\
\ion{Ar}{1} 1066&1066.686&1066.660& 0.00002&$ 105$&$ 11$&$ 176$&$ 48$&$ 110$&  9\\
H$_2$&1066.907&1066.900& 0.00001&$  54$&$  9$&$  94$&$ 39$&$  56$&  9\\
H$_2$&1067.460&1067.479&-0.00002&$  34$&$  8$&$  54$&$ 36$&$  35$&  7\\
\ion{C}{3} 977&1068.800& 977.020& 0.09394&$  80$&$  9$& \nodata & \nodata &$  80$&  9\\
\ion{H}{1} 972&1068.800& 972.537& 0.09898&$  80$&$  9$& \nodata & \nodata &$  80$&  9\\
\ion{H}{1} 1025&1069.017&1025.722& 0.04221&$ 222$&$ 11$& \nodata & \nodata &$ 222$& 11\\
\ion{C}{3} 977&1069.728& 977.020& 0.09489&$ 243$&$ 13$& \nodata & \nodata &$ 243$& 13\\
H$_2$&1070.158&1070.141& 0.00002&$  43$&$  9$&$ -37$&$ 42$&$  40$&  9\\
\ion{H}{1} 1025&1071.291&1025.722& 0.04443&$  17$&$ 14$& \nodata & \nodata &$  17$& 14\\
\ion{H}{1} 1025&1073.575&1025.722& 0.04665&$  61$&$ 15$& \nodata & \nodata &$  61$& 15\\
\ion{O}{6} 1031&1075.703&1031.926& 0.04242&$ 190$&$ 18$& \nodata & \nodata &$ 190$& 18\\
H$_2$&1077.148&1076.992& 0.00014&$  62$&$ 12$&$ 135$&$ 37$&$  68$& 11\\
H$_2$&1077.696&1077.700&-0.00000&$  72$&$ 10$&$ 158$&$ 31$&$  80$& 10\\
H$_2$&1078.920&1078.927&-0.00001&$  74$&$ 10$&$ 161$&$ 34$&$  81$& 10\\
H$_2$&1079.206&1079.226&-0.00002&$  34$&$ 10$&$ 122$&$ 30$&$  43$& 10\\
H$_2$&1081.243&1081.267&-0.00002&$ 107$&$ 12$&$ 118$&$ 38$&$ 108$& 12\\
H$_2$&1081.552&1081.713&-0.00015&$ 181$&$ 16$&$ 253$&$ 45$&$ 189$& 15\\
\ion{O}{6} 1037&1081.585&1037.617& 0.04237&$ 173$&$ 15$& \nodata & \nodata &$ 173$& 15\\
\ion{Fe}{2} 1081&1081.828&1081.875&-0.00004&$  92$&$ 13$&$  95$&$ 39$&$  93$& 13\\
\ion{N}{2} 1083&1084.050&1083.990& 0.00006&$ 464$&$ 60$& \nodata & \nodata &$ 464$& 60\\
\ion{H}{1} 949&1087.773& 949.743& 0.14533&$  89$&$ 16$& \nodata & \nodata &$  89$& 16\\
\ion{H}{1} 1025&1092.106&1025.722& 0.06472&$ 143$&$ 16$& \nodata & \nodata &$ 143$& 16\\
H$_2$&1092.106&1092.195&-0.00008&$ 104$&$  9$& \nodata & \nodata &$ 104$&  9\\
H$_2$&1092.659&1092.732&-0.00007&$  80$&$  9$& \nodata & \nodata &$  80$&  9\\
\ion{H}{1} 917&1092.850& 917.181& 0.19153&$   1$&$ 11$& \nodata & \nodata &$   1$& 11\\
\ion{H}{1} 918&1093.972& 918.129& 0.19152&$  70$&$ 11$& \nodata & \nodata &$  70$& 11\\
H$_2$&1093.989&1094.052&-0.00006&$  83$&$ 10$& \nodata & \nodata &$  83$& 10\\
H$_2$&1094.191&1094.244&-0.00005&$  30$&$ 10$& \nodata & \nodata &$  30$& 10\\
\ion{H}{1} 919&1095.548& 919.351& 0.19165&$  58$&$ 12$&$  15$&$ 13$&$  38$&  9\\
H$_2$&1096.350&1096.438&-0.00008&$  19$&$  9$&$  48$&$  9$&$  33$&  6\\
\ion{Fe}{2} 1096&1096.805&1096.877&-0.00007&$ 214$&$ 13$&$ 166$&$ 15$&$ 194$& 10\\
\ion{H}{1} 920&1097.359& 920.963& 0.19153&$  39$&$ 11$&$  43$&$ 12$&$  41$&  8\\
\ion{O}{6} 1031&1098.653&1031.926& 0.06466&$  33$&$ 14$&$  63$&$ 16$&$  47$& 11\\
\ion{H}{1} 923&1099.999& 923.150& 0.19157&$  32$&$  9$&$  29$&$ 11$&$  31$&  7\\
\ion{H}{1} 926&1103.694& 926.226& 0.19160&$  41$&$ 10$&$  40$&$ 12$&$  41$&  8\\
\ion{O}{6} 1037&1104.712&1037.617& 0.06466&$  28$&$ 13$&$  61$&$ 15$&$  42$& 10\\
H$_2$&1108.018&1108.127&-0.00010&$  44$&$  8$&$  50$&$  9$&$  47$&  6\\
H$_2$&1108.590&1108.633&-0.00004&$  29$&$ 13$&$  72$&$ 15$&$  47$& 10\\
\ion{H}{1} 930&1109.022& 930.748& 0.19154&$  43$&$ 10$&$  62$&$ 12$&$  51$&  8\\
H$_2$&1110.005&1110.063&-0.00005&$  93$&$  8$&$  67$&$ 10$&$  83$&  6\\
\ion{H}{1} 949&1110.566& 949.743& 0.16933&$  -6$&$ 13$&$  49$&$ 15$&$  18$& 10\\
\ion{Fe}{2} 1112&1111.979&1112.048&-0.00006&$  59$&$ 13$&$  56$&$ 15$&$  58$& 10\\
H$_2$&1112.444&1112.495&-0.00005&$  53$&$ 10$&$  50$&$ 12$&$  52$&  8\\
\ion{H}{1} 972&1113.814& 972.537& 0.14527&$ 315$&$ 14$&$ 350$&$ 16$&$ 330$& 11\\
\ion{H}{1} 937&1117.441& 937.803& 0.19155&$  67$&$ 10$&$  91$&$ 11$&$  77$&  7\\
\ion{C}{3} 977&1118.923& 977.020& 0.14524&$  71$&$ 13$&$  59$&$ 15$&$  66$& 10\\
\ion{Fe}{2} 1121&1122.053&1121.975& 0.00007&$ 411$&$ 16$&$ 422$&$ 17$&$ 416$& 12\\
\ion{H}{1} 1025&1122.053&1025.722& 0.09392&$ 376$&$ 12$&$ 374$&$ 13$&$ 375$&  9\\
\ion{Fe}{3} 1122&1122.514&1122.526&-0.00001&$ 109$&$  9$&$  88$&$ 10$&$ 100$&  7\\
\ion{H}{1} 1025&1122.993&1025.722& 0.09483&$ 516$&$ 13$&$ 553$&$ 14$&$ 533$&  9\\
\ion{Fe}{2} 1125&1125.413&1125.448&-0.00003&$ 143$&$ 14$&$ 111$&$ 16$&$ 129$& 11\\
\ion{H}{1} 1025&1127.186&1025.722& 0.09892&$ 108$&$ 10$&$  92$&$ 12$&$ 101$&  8\\
\ion{O}{6} 1031&1129.855&1031.926& 0.09490&$  81$&$ 19$&$ 115$&$ 21$&$  97$& 14\\
\ion{H}{1} 949&1131.691& 949.743& 0.19158&$ 140$&$ 11$&$ 142$&$ 12$&$ 141$&  8\\
\ion{Fe}{2} 1133&1133.623&1133.665&-0.00004&$  76$&$  9$&$  28$&$ 11$&$  57$&  7\\
\ion{N}{1} 1134a&1134.065&1134.165&-0.00009&$ 197$&$ 13$& \nodata & \nodata &$ 197$& 13\\
\ion{N}{1} 1134b&1134.338&1134.415&-0.00007&$ 178$&$ 15$& \nodata & \nodata &$ 178$& 15\\
\ion{N}{1} 1134c&1134.955&1134.980&-0.00002&$ 139$&$ 20$& \nodata & \nodata &$ 139$& 20\\
\ion{O}{6} 1037&1135.955&1037.617& 0.09477&$  35$&$ 17$&$  49$&$ 19$&$  42$& 13\\
\ion{H}{1} 972&1137.345& 972.537& 0.16946&$  27$&$ 14$&$  21$&$ 16$&$  24$& 11\\
\ion{Fe}{2} 1142&1142.302&1142.366&-0.00006&$  72$&$ 17$&$  64$&$ 14$&$  68$& 11\\
\ion{Fe}{2} 1143&1143.211&1143.226&-0.00001&$ 130$&$ 19$&$ 139$&$ 15$&$ 135$& 12\\
\ion{Fe}{2} 1144&1144.867&1144.938&-0.00006&$ 252$&$ 18$&$ 241$&$ 14$&$ 245$& 11\\
\ion{H}{1} 1025&1152.203&1025.722& 0.12331&$  -4$&$ 19$&$  20$&$ 15$&$  11$& 12\\
\ion{P}{2} 1152&1152.778&1152.818&-0.00003&$  72$&$ 18$&$  81$&$ 15$&$  77$& 12\\
\ion{H}{1} 1025&1154.594&1025.722& 0.12564&$  49$&$ 15$&$  57$&$ 67$&$  34$& 11\\
\ion{H}{1} 972&1158.832& 972.537& 0.19156&$ 199$&$ 14$&$ 158$&$ 48$&$ 174$& 10\\
\ion{H}{1} 972&1159.471& 972.537& 0.19221&$  23$&$ 14$&$ -97$&$ 47$&$  23$& 10\\
\ion{H}{1} 972&1160.112& 972.537& 0.19287&$  23$&$ 15$&$  28$&$ 43$&$   3$& 11\\
\ion{C}{3} 977&1164.212& 977.020& 0.19160&$  49$&$ 13$&$  74$&$ 34$&$  48$&  9\\
\ion{H}{1} 937&1171.068& 937.803& 0.24873&$   8$&$ 14$&$   7$&$ 33$&$  -2$& 10\\
\ion{H}{1} 1025&1174.796&1025.722& 0.14534&$ 532$&$ 17$&$ 572$&$ 35$&$ 560$& 11\\
\ion{O}{6} 1031&1181.859&1031.926& 0.14529&$ 124$&$ 26$&$  40$&$ 41$&$ 100$& 22\\
\ion{H}{1} 949&1185.867& 949.743& 0.24862&$  37$&$ 18$&$  22$&$ 24$&$  32$& 14\\
\ion{C}{2} 1036&1186.961&1036.337& 0.14534&$ -32$&$ 21$&$ -17$&$ 21$&$ -25$& 15\\
\ion{H}{1} 1025&1188.176&1025.722& 0.15838&$  95$&$ 20$& \nodata & \nodata &$  95$& 20\\
\ion{O}{6} 1037&1188.285&1037.617& 0.14521&$ 111$&$ 30$& \nodata & \nodata &$ 111$& 30\\
\cutinhead{STIS}
\ion{H}{1} 949&1189.163& 949.743& 0.25209&$   5$&$ 16$& \nodata & \nodata &$   5$& 16\\
\ion{Si}{2} 1190&1190.423&1190.415& 0.00001&$ 423$&$ 23$& \nodata & \nodata &$ 423$& 23\\
\ion{H}{1} 972&1190.892& 972.537& 0.22452&$  49$&$ 20$& \nodata & \nodata &$  49$& 20\\
\ion{H}{1} 972&1191.828& 972.537& 0.22548&$ -34$&$ 20$& \nodata & \nodata &$ -34$& 20\\
\ion{Si}{2} 1193&1193.302&1193.290& 0.00001&$ 378$&$ 25$& \nodata & \nodata &$ 378$& 25\\
\ion{C}{3} 977&1197.488& 977.020& 0.22565&$  17$&$ 19$& \nodata & \nodata &$  17$& 19\\
\ion{H}{1} 1025&1199.538&1025.722& 0.16946&$ 280$&$ 14$& \nodata & \nodata &$ 280$& 14\\
\ion{N}{1} 1199&1199.538&1199.550&-0.00001&$ 307$&$ 17$& \nodata & \nodata &$ 307$& 17\\
\ion{N}{1} 1200&1200.221&1200.223&-0.00000&$ 346$&$ 17$& \nodata & \nodata &$ 346$& 17\\
\ion{N}{1} 1200c&1200.704&1200.710&-0.00001&$ 341$&$ 18$& \nodata & \nodata &$ 341$& 18\\
\ion{Si}{3} 1206&1206.503&1206.500& 0.00000&$ 378$&$ 20$& \nodata & \nodata &$ 378$& 20\\
\ion{H}{1} 972&1217.672& 972.537& 0.25206&$ 148$&$126$& \nodata & \nodata &$ 148$&126\\
\ion{H}{1} 1215&1220.992&1215.670& 0.00438&$ 327$&$ 25$& \nodata & \nodata &$ 327$& 25\\
\ion{H}{1} 972&1221.340& 972.537& 0.25583&$  -6$&$ 13$& \nodata & \nodata &$  -6$& 13\\
\ion{H}{1} 1025&1222.260&1025.722& 0.19161&$ 235$&$ 14$& \nodata & \nodata &$ 235$& 14\\
\ion{H}{1} 1025&1223.148&1025.722& 0.19247&$  41$&$ 15$& \nodata & \nodata &$  41$& 15\\
\ion{H}{1} 1025&1223.654&1025.722& 0.19297&$  45$&$ 11$& \nodata & \nodata &$  45$& 11\\
\ion{O}{6} 1031&1229.656&1031.926& 0.19161&$  68$&$ 14$& \nodata & \nodata &$  68$& 14\\
\ion{C}{2} 1036&1234.903&1036.337& 0.19160&$  -8$&$ 12$& \nodata & \nodata &$  -8$& 12\\
\ion{O}{6} 1037&1236.333&1037.617& 0.19151&$ -13$&$ 11$& \nodata & \nodata &$ -13$& 11\\
\ion{H}{1} 1215&1237.389&1215.670& 0.01787&$  23$&$ 11$& \nodata & \nodata &$  23$& 11\\
\ion{N}{5} 1238&1238.752&1238.821&-0.00006&$  -5$&$ 19$& \nodata & \nodata &$  -5$& 19\\
\ion{N}{5} 1242&1242.819&1242.804& 0.00001&$  31$&$ 14$& \nodata & \nodata &$  31$& 14\\
\ion{S}{2} 1250&1250.565&1250.584&-0.00002&$ 160$&$ 11$& \nodata & \nodata &$ 160$& 11\\
\ion{S}{2} 1253&1253.784&1253.811&-0.00002&$ 209$&$ 11$& \nodata & \nodata &$ 209$& 11\\
\ion{H}{1} 1025&1256.022&1025.722& 0.22452&$  60$&$ 11$& \nodata & \nodata &$  60$& 11\\
\ion{H}{1} 1025&1257.034&1025.722& 0.22551&$  66$&$ 11$& \nodata & \nodata &$  66$& 11\\
\ion{S}{2} 1259&1259.521&1259.519& 0.00000&$ 222$&$ 10$& \nodata & \nodata &$ 222$& 10\\
\ion{Si}{2} 1260&1260.407&1260.422&-0.00001&$ 497$&$ 14$& \nodata & \nodata &$ 497$& 14\\
\ion{O}{6} 1031&1264.729&1031.926& 0.22560&$  52$&$ 12$& \nodata & \nodata &$  52$& 12\\
\ion{H}{1} 1025&1265.824&1025.722& 0.23408&$   4$&$  9$& \nodata & \nodata &$   4$&  9\\
\ion{O}{6} 1031&1266.603&1031.926& 0.22742&$  38$&$  8$& \nodata & \nodata &$  38$&  8\\
\ion{H}{1} 1215&1266.994&1215.670& 0.04222&$ 408$&$ 13$& \nodata & \nodata &$ 408$& 13\\
\ion{H}{1} 1025&1268.477&1025.722& 0.23667&$   3$&$ 10$& \nodata & \nodata &$   3$& 10\\
\ion{H}{1} 1215&1269.721&1215.670& 0.04446&$ 149$&$ 10$& \nodata & \nodata &$ 149$& 10\\
\ion{O}{6} 1037&1271.803&1037.617& 0.22570&$  99$&$ 12$& \nodata & \nodata &$  99$& 12\\
\ion{H}{1} 1215&1272.299&1215.670& 0.04658&$ 228$&$ 12$& \nodata & \nodata &$ 228$& 12\\
\ion{O}{6} 1037&1273.604&1037.617& 0.22743&$  11$&$  9$& \nodata & \nodata &$  11$&  9\\
\ion{H}{1} 1025&1280.893&1025.722& 0.24877&$  75$&$  7$& \nodata & \nodata &$  75$&  7\\
\ion{H}{1} 1025&1283.332&1025.722& 0.25115&$   6$&$ 14$& \nodata & \nodata &$   6$& 14\\
\ion{H}{1} 1025&1284.358&1025.722& 0.25215&$ 220$&$ 11$& \nodata & \nodata &$ 220$& 11\\
\ion{H}{1} 1025&1285.027&1025.722& 0.25280&$  53$&$ 11$& \nodata & \nodata &$  53$& 11\\
\ion{H}{1} 1025&1286.266&1025.722& 0.25401&$  15$&$ 14$& \nodata & \nodata &$  15$& 14\\
\ion{H}{1} 1215&1287.019&1215.670& 0.05869&$  86$&$ 10$& \nodata & \nodata &$  86$& 10\\
\ion{H}{1} 1215&1288.219&1215.670& 0.05968&$  72$&$  8$& \nodata & \nodata &$  72$&  8\\
\ion{H}{1} 1215&1294.341&1215.670& 0.06471&$ 265$&$ 14$& \nodata & \nodata &$ 265$& 14\\
\ion{P}{2} 1301&1301.843&1301.874&-0.00002&$  10$&$  9$& \nodata & \nodata &$  10$&  9\\
\ion{O}{1} 1302&1302.210&1302.168& 0.00003&$ 442$&$ 13$& \nodata & \nodata &$ 442$& 13\\
\ion{Si}{2} 1304&1304.332&1304.370&-0.00003&$ 336$&$ 13$& \nodata & \nodata &$ 336$& 13\\
\ion{Ni}{2} 1317&1317.251&1317.217& 0.00003&$  49$&$ 11$& \nodata & \nodata &$  49$& 11\\
\ion{Si}{3} 1206&1320.956&1206.500& 0.09487&$ 172$&$  8$& \nodata & \nodata &$ 172$&  8\\
\ion{H}{1} 1215&1329.943&1215.670& 0.09400&$ 439$&$ 11$& \nodata & \nodata &$ 439$& 11\\
\ion{H}{1} 1215&1331.004&1215.670& 0.09487&$ 679$&$ 12$& \nodata & \nodata &$ 679$& 12\\
\ion{C}{2} 1334&1334.503&1334.532&-0.00002&$ 486$&$ 12$& \nodata & \nodata &$ 486$& 12\\
\ion{C}{2} 1335&1335.666&1335.708&-0.00003&$ 166$&$  7$& \nodata & \nodata &$ 166$&  7\\
\ion{H}{1} 1215&1335.915&1215.670& 0.09891&$ 362$&$  7$& \nodata & \nodata &$ 362$&  7\\
\ion{C}{2} 1334&1340.382&1334.532& 0.00438&$   0$&$ 16$& \nodata & \nodata &$   0$& 16\\
\ion{O}{1} 1302&1357.231&1302.168& 0.04229&$  -2$&$ 13$& \nodata & \nodata &$  -2$& 13\\
\ion{H}{1} 1215&1361.546&1215.670& 0.12000&$  11$&$  8$& \nodata & \nodata &$  11$&  8\\
\ion{H}{1} 1215&1365.581&1215.670& 0.12332&$ 135$&$ 13$& \nodata & \nodata &$ 135$& 13\\
\ion{H}{1} 1215&1368.425&1215.670& 0.12565&$  66$&$ 10$& \nodata & \nodata &$  66$& 10\\
\ion{Ni}{2} 1370&1370.164&1370.131& 0.00002&$  55$&$  9$& \nodata & \nodata &$  55$&  9\\
\ion{Si}{2} 1260&1380.036&1260.422& 0.09490&$  31$&$ 11$& \nodata & \nodata &$  31$& 11\\
\ion{O}{1} 1302&1386.385&1302.168& 0.06467&$ -12$&$ 13$& \nodata & \nodata &$ -12$& 13\\
\ion{C}{2} 1334&1390.909&1334.532& 0.04224&$   5$&$ 14$& \nodata & \nodata &$   5$& 14\\
\ion{H}{1} 1215&1392.344&1215.670& 0.14533&$ 868$&$ 15$& \nodata & \nodata &$ 868$& 15\\
\ion{Si}{4} 1393&1393.772&1393.755& 0.00001&$ 232$&$ 12$& \nodata & \nodata &$ 232$& 12\\
\ion{Si}{4} 1402&1402.808&1402.770& 0.00003&$ 120$&$ 12$& \nodata & \nodata &$ 120$& 12\\
\ion{H}{1} 1215&1408.170&1215.670& 0.15835&$  71$&$ 11$& \nodata & \nodata &$  71$& 11\\
\ion{H}{1} 1215&1421.538&1215.670& 0.16935&$ 212$&$ 13$& \nodata & \nodata &$ 212$& 13\\
\ion{O}{1} 1302&1425.705&1302.168& 0.09487&$  -2$&$ 18$& \nodata & \nodata &$  -2$& 18\\
\ion{Si}{3} 1206&1437.696&1206.500& 0.19163&$  22$&$  8$& \nodata & \nodata &$  22$&  8\\
\ion{H}{1} 1215&1448.599&1215.670& 0.19161&$ 401$&$ 10$& \nodata & \nodata &$ 401$& 10\\
\ion{H}{1} 1215&1449.602&1215.670& 0.19243&$ 222$&$  8$& \nodata & \nodata &$ 222$&  8\\
\ion{H}{1} 1215&1450.246&1215.670& 0.19296&$ 220$&$  8$& \nodata & \nodata &$ 220$&  8\\
\ion{H}{1} 1215&1452.110&1215.670& 0.19449&$  -5$&$ 10$& \nodata & \nodata &$  -5$& 10\\
\ion{C}{2} 1334&1460.006&1334.532& 0.09402&$  -5$&$ 14$& \nodata & \nodata &$  -5$& 14\\
\ion{C}{2} 1334&1461.189&1334.532& 0.09491&$  73$&$ 18$& \nodata & \nodata &$  73$& 18\\
\ion{H}{1} 1215&1488.674&1215.670& 0.22457&$ 298$&$ 13$& \nodata & \nodata &$ 298$& 13\\
\ion{H}{1} 1215&1489.866&1215.670& 0.22555&$ 324$&$ 13$& \nodata & \nodata &$ 324$& 13\\
\ion{O}{1} 1302&1491.499&1302.168& 0.14540&$ -42$&$ 16$& \nodata & \nodata &$ -42$& 16\\
\ion{H}{1} 1215&1492.260&1215.670& 0.22752&$  54$&$ 14$& \nodata & \nodata &$  54$& 14\\
\ion{H}{1} 1215&1500.185&1215.670& 0.23404&$  10$&$ 13$& \nodata & \nodata &$  10$& 13\\
\ion{H}{1} 1215&1503.392&1215.670& 0.23668&$  60$&$ 11$& \nodata & \nodata &$  60$& 11\\
\ion{H}{1} 1215&1507.475&1215.670& 0.24004&$  81$&$  9$& \nodata & \nodata &$  81$&  9\\
\ion{H}{1} 1215&1518.071&1215.670& 0.24875&$ 263$&$ 14$& \nodata & \nodata &$ 263$& 14\\
\ion{H}{1} 1215&1520.922&1215.670& 0.25110&$ 201$&$ 16$& \nodata & \nodata &$ 201$& 16\\
\ion{H}{1} 1215&1522.250&1215.670& 0.25219&$ 447$&$ 12$& \nodata & \nodata &$ 447$& 12\\
\ion{H}{1} 1215&1523.069&1215.670& 0.25286&$ 281$&$ 12$& \nodata & \nodata &$ 281$& 12\\
\ion{H}{1} 1215&1524.594&1215.670& 0.25412&$ 227$&$ 16$& \nodata & \nodata &$ 227$& 16\\
\ion{Si}{4} 1393&1525.891&1393.755& 0.09481&$   8$&$ 12$& \nodata & \nodata &$   8$& 12\\
\ion{Si}{2} 1526&1526.719&1526.707& 0.00001&$ 396$&$ 12$& \nodata & \nodata &$ 396$& 12\\
\ion{C}{2} 1334&1528.538&1334.532& 0.14537&$  -6$&$ 14$& \nodata & \nodata &$  -6$& 14\\
\ion{Si}{4} 1402&1535.924&1402.770& 0.09492&$   3$&$ 14$& \nodata & \nodata &$   3$& 14\\
\ion{C}{4} 1548&1548.231&1548.195& 0.00002&$ 290$&$ 12$& \nodata & \nodata &$ 290$& 12\\
\ion{C}{4} 1550&1550.798&1550.770& 0.00002&$ 195$&$ 11$& \nodata & \nodata &$ 195$& 11\\
\ion{O}{1} 1302&1551.678&1302.168& 0.19161&$  -9$&$ 12$& \nodata & \nodata &$  -9$& 12\\
\ion{C}{4} 1548&1555.011&1548.195& 0.00440&$  44$&$ 13$& \nodata & \nodata &$  44$& 13\\
\ion{C}{4} 1550&1557.529&1550.770& 0.00436&$  14$&$ 14$& \nodata & \nodata &$  14$& 14\\
\ion{C}{1} 1560&1560.317&1560.309& 0.00000&$  30$&$ 11$& \nodata & \nodata &$  30$& 11\\
\ion{C}{4} 1548&1582.908&1548.195& 0.02242&$  14$&$ 16$& \nodata & \nodata &$  14$& 16\\
\ion{C}{4} 1550&1585.519&1550.770& 0.02241&$   4$&$ 14$& \nodata & \nodata &$   4$& 14\\
\ion{C}{2} 1334&1590.354&1334.532& 0.19169&$ -22$&$ 14$& \nodata & \nodata &$ -22$& 14\\
\ion{O}{1} 1302&1596.002&1302.168& 0.22565&$  15$&$ 19$& \nodata & \nodata &$  15$& 19\\
\ion{Fe}{2} 1608&1608.463&1608.451& 0.00001&$ 392$&$ 18$& \nodata & \nodata &$ 392$& 18\\
\ion{C}{4} 1548&1613.597&1548.195& 0.04224&$  88$&$ 22$& \nodata & \nodata &$  88$& 22\\
\ion{C}{4} 1550&1616.217&1550.770& 0.04220&$  24$&$ 19$& \nodata & \nodata &$  24$& 19\\
\ion{C}{4} 1548&1648.349&1548.195& 0.06469&$   9$&$ 25$& \nodata & \nodata &$   9$& 25\\
\ion{C}{4} 1550&1650.905&1550.770& 0.06457&$   2$&$ 26$& \nodata & \nodata &$   2$& 26\\
\ion{Al}{2} 1670&1670.786&1670.787&-0.00000&$ 398$&$ 16$& \nodata & \nodata &$ 398$& 16\\
\ion{C}{4} 1548&1693.574&1548.195& 0.09390&$ -20$&$ 32$& \nodata & \nodata &$ -20$& 32\\
\ion{C}{4} 1548&1694.987&1548.195& 0.09481&$  43$&$ 37$& \nodata & \nodata &$  43$& 37\\
\ion{C}{4} 1550&1696.467&1550.770& 0.09395&$ -49$&$ 28$& \nodata & \nodata &$ -49$& 28\\
\ion{C}{4} 1550&1697.842&1550.770& 0.09484&$  -9$&$ 33$& \nodata & \nodata &$  -9$& 33\\
\enddata
\tablecomments{Note that the list is incomplete for wavelengths $< 1000$\AA\ where the data has poor S/N and significant line blending.
Columns 4,5 (6,7) refer to the SiC 1B (SiC 2A) channel for 905$ < \lambda < 1005\,$\AA; LiF1A for 990$ < \lambda < 1090\,$\AA; LiF 1B (LiF 2A) for 1088$ < \lambda < 1188$\AA; and STIS E140M for $\lambda > 1188\,$\AA.}
\end{deluxetable}

